Paths Explored, Paths Omitted, Paths Obscured: Decision Points & Selective Reporting in End-to-End Data Analysis

Drawing reliable inferences from data involves many, sometimes arbitrary, decisions across phases of data collection, wrangling, and modeling. As different choices can lead to diverging conclusions, understanding how researchers make analytic decisions is important for supporting robust and replicable analysis. In this study, we pore over nine published research studies and conduct semi-structured interviews with their authors. We observe that researchers often base their decisions on methodological or theoretical concerns, but subject to constraints arising from the data, expertise, or perceived interpretability. We confirm that researchers may experiment with choices in search of desirable results, but also identify other reasons why researchers explore alternatives yet omit findings. In concert with our interviews, we also contribute visualizations for communicating decision processes throughout an analysis. Based on our results, we identify design opportunities for strengthening end-to-end analysis, for instance via tracking and meta-analysis of multiple decision paths.

==> conclusion.tex <==
\section{Conclusion}

In this work, we scrutinized nine published studies in various fields and interviewed their authors to discuss decision points in analysis processes.
We presented common rationales for analytic decisions and how researchers suppressed tradeoffs among options.
We also discussed why researchers carried out alternative analyses and how researchers decided to omit findings in research reports.
Finally, we developed visualizations for better structuring and communicating analysis processes.
We hope our results will provide useful information on how data analysis process in academic research could be strengthened and will help inspire new research directions.

